V1298 Tau with TESS: Updated Ephemerides, Radii, and Period Constraints from a Second Transit of V1298 Tau e

V1298 Tau is a young (20-30 Myr) solar-mass K star hosting four transiting exoplanets with sizes between 0.5 - 0.9 $R_J$. Given the system's youth, it provides a unique opportunity to understand the evolution of planetary radii at different separations in the same stellar environment. V1298 Tau was originally observed 6 years ago during K2 Campaign 4. Now, V1298 Tau has been re-observed during the extended mission of NASA's Transiting Exoplanet Survey Satellite (TESS). Here, we present new photometric observations of V1298 Tau from the 10-minute TESS Full-Frame Images. We use the TESS data to update the ephemerides for V1298 Tau bcde as well as compare newly observed radii to those measured from the K2 light curve, finding shallower transits for V1298 Tau bcd in the redder TESS bandpass at the $1-2\sigma$ level. We suspect the difference in radii is due to starspot-crossing events or contamination from nearby faint stars on the same pixels as V1298 Tau. Additionally, we catch a second transit of V1298 Tau e and present a new method for deriving the marginalized posterior probability of a planet's period from two transits observed years apart. We find the highest probability period for V1298 Tau e to be in a near 2:1 mean motion resonance with V1298 Tau b which, if confirmed, could make V1298 Tau bcde a 4 planet resonant chain. V1298 Tau is the target of several ongoing and future observations. These updated ephemerides will be crucial for scheduling future transit observations and interpreting future Doppler tomographic or transmission spectroscopy signals.

==> listofitems.tex <==
% !TeX encoding = ISO-8859-1
% Ce fichier contient le code de l'extension "listofitems"
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                    %
\def\loiname                 {listofitems}                           %
\def\loiver                      {1.63}                              %
%                                                                    %
\def\loidate                  {2019/08/21}                           %
%                                                                    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                    %
% Author     : Christian Tellechea, Steven B. Segletes (contributor) %
% Status     : Maintained                                            %
% Maintainer : Christian Tellechea                                   %
% Email      : unbonpetit@netc.fr                                    %
%              steven.b.segletes.civ@mail.mil                        %
% Package URL: https://www.ctan.org/pkg/listofitems                  %
% Bug tracker: https://framagit.org/unbonpetit/listofitems/issues    %
% Repository : https://framagit.org/unbonpetit/listofitems/tree/master
% Copyright  : Christian Tellechea 2016-2019                         %
% Licence    : Released under the LaTeX Project Public License v1.3c %
%              or later, see http://www.latex-project.org/lppl.txt   %
% Files      : 1) listofitems.tex                                    %
%              2) listofitems.sty                                    %
%              3) listofitems-fr.tex                                 %
%              4) listofitems-fr.pdf                                 %
%              5) listofitems-en.tex                                 %
%              6) listofitems-en.pdf                                 %
%              7) README                                             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\expandafter\edef\csname loi_restorecatcode\endcsname{\catcode\number`\_=\number\catcode`\_\relax}
\catcode`\_11

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%% gestion des erreurs + annonce package %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\unless\ifdefined\loi_fromsty
	\immediate\write -1 {Package: \loidate\space v\loiver\space Grab items in lists using user-specified sep char (CT)}%
\fi

\ifdefined\PackageError
	\def\loi_error#1{\PackageError\loiname{#1}{Read the \loiname\space manual}}% pour LaTeX
\else
	\def\loi_error#1{\errmessage{Package \loiname\space Error: #1^^J}}% pour TeX
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% verification des prerequis %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\loi_checkprimitive#1#2#3{% Verifie que #1 est une primitive et sinon, emet le message #2 et execute #3
	\begingroup
		\edef\__tempa{\meaning#1}\edef\__tempb{\string#1}\expandafter
	\endgroup
	\ifx\__tempa\__tempb\else
		\loi_error{#2}%
		\def\loi_temp{#3}%
		\loi_restorecatcode\expandafter\loi_temp
	\fi
}
\loi_checkprimitive\eTeXversion
	{You are not using an eTeX engine, listofitems cannot work.}
	{\endinput}%
\loi_checkprimitive\expanded
	{the \string\expanded\space primitive is not provided by your TeX engine, listofitems v\loiver\space cannot work: loading listofitems v1.61}
	{\input listofitemsold.tex\relax\endinput}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% macros auxiliaires %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\loi_quark{\loi_quark}
\long\def\loi_identity#1{#1}
\long\def\loi_gobarg#1{}
\long\def\loi_first#1#2{#1}
\long\def\loi_second#1#2{#2}
\long\def\loi_firsttonil#1#2\_nil{#1}
\long\def\loi_antefi#1#2\fi{#2\fi#1}
\long\def\loi_exparg#1#2{\expandafter\loi_exparg_a\expandafter{#2}{#1}}% \loi_exparg{<a>}{<b>} devient <a>{<*b>}
\long\def\loi_exparg_a#1#2{#2{#1}}
\long\def\loi_expafter#1#2{\expandafter\loi_expafter_a\expandafter{#2}{#1}}% \loi_expafter{<a>}{<b>} devient <a><*b>
\long\def\loi_expafter_a#1#2{#2#1}
\def\loi_macroname{\loi_ifinrange\escapechar[[0:255]]{\expandafter\loi_gobarg}{}\string}
\def\loi_argcsname#1#{\loi_argcsname_a{#1}}
\def\loi_argcsname_a#1#2{\loi_expafter{#1}{\csname#2\endcsname}}
\long\def\loi_addtomacro#1#2{\loi_exparg{\def#1}{#1#2}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%% macros de test %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\long\def\loi_ifnum#1{\ifnum#1\expandafter\loi_first\else\expandafter\loi_second\fi}
\long\def\loi_ifx#1{\ifx#1\expandafter\loi_first\else\expandafter\loi_second\fi}
\long\def\loi_ifempty#1{\loi_exparg\loi_ifx{\expandafter\relax\detokenize{#1}\relax}}
\def\loi_ifstar#1#2{\def\loi_ifstar_a{\loi_ifx{*\loi_nxttok}{\loi_first{#1}}{#2}}\futurelet\loi_nxttok\loi_ifstar_a}
\edef\loi_escapechar{\expandafter\loi_gobarg\string\\}
\long\def\loi_ifcsexpandable#1{% #1 est-il constitue d'une seule sc _developpable_ ?
	\loi_ifempty{#1}
		{\loi_second
		}
		{\loi_ifspacefirst{#1}
			{\loi_second% si espace en 1er, faux
			}
			{\csname loi_\if\loi_escapechar\expandafter\loi_firsttonil\detokenize{#1}\_nil first\else second\fi\endcsname
				{\loi_exparg\loi_ifempty{\loi_gobarg#1}% 1 seul arg commeneant par "\" ?
					{\def\loi_tempa{#1}\loi_exparg{\def\loi_tempb}{#1}% est-il developpable ?
					\expandafter\unless\loi_ifx{\loi_tempa\loi_tempb}%
					}
					{\loi_second
					}%
				}
				{\loi_second
				}%
			}%
		}%
}
\def\loi_ifinrange#1[[#2:#3]]{\expandafter\unless\loi_ifnum{\numexpr(#1-#2)*(#1-#3)>0 }}
\def\loi_ifstring#1#2{% si la chaine #1 est contenue dans #2
	\def\loi_ifstring_a##1#1##2\_nil{\loi_ifempty{##2}\loi_second\loi_first}%
	\loi_ifstring_a#2#1\_nil% appel de la macro auxiliaire
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% macro \loi_foreach %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcount\loi_cnt_foreach_nest \loi_cnt_foreach_nest=0
\def\end_foreach{\end_foreach}
\def\loi_def_foreachsep#1{%
	\long\def\loi_foreach##1\in##2##3{%
		\global\advance\loi_cnt_foreach_nest1
		\loi_argcsname\def{loop_code_\number\loi_cnt_foreach_nest}{##3}%
		\loi_foreach_a##1##2#1\end_foreach#1%
		\loi_argcsname\let{loop_code_\number\loi_cnt_foreach_nest}\empty
		\global\advance\loi_cnt_foreach_nest-1
	}%
	\long\def\loi_foreach_a##1##2#1{%
		\def##1{##2}%
		\loi_ifx{\end_foreach##1}
			{}
			{\csname loop_code_\number\loi_cnt_foreach_nest\endcsname% execute le code
			\loi_foreach_a##1%
			}%
	}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% macros gerant l'appariement %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\long\def\defpair#1{%
	\let\loi_listofpair\empty
	\loi_ifempty{#1}
		{}
		{\defpair_a{}#1\loi_quark\loi_quark}%
}
\long\def\defpair_a#1#2#3{%
	\loi_ifx{\loi_quark#2}
		{\def\loi_sanitizelist##1,\_nil{\def\loi_listofpair{##1}}%
		\loi_sanitizelist#1\_nil
		}
		{\loi_if_validpair#2#3%
			{\long\def\loi_paired_a{#2}\long\def\loi_paired_b{#3}%
			\loi_ifx{\loi_paired_a\loi_paired_b}
				{\loi_error{Paired tokens must not be equal, the pair \detokenize{#2#3} is ignored}%
				\defpair_a{#1}%
				}
				{\defpair_a{#1#2#3,}%
				}%
			}
			{\loi_error{Invalid paired tokens, the pair "\detokenize{#2}" and "\detokenize{#3}" is ignored}%
			\defpair_a{#1}%
			}%
		}%
}
\long\def\loi_if_validpair#1#2{%
	\def\loi_validpair{1}%
	\loi_if_invalid_pairtoken{#1}{\def\loi_validpair{0}}%
	\loi_if_invalid_pairtoken{#2}{\def\loi_validpair{0}}%
	\loi_ifnum{\loi_validpair=1 }
}
\long\def\loi_if_invalid_pairtoken#1{%
	\loi_ifempty{#1}
		{\loi_identity
		}
		{\loi_ifspacefirst{#1}
			{\loi_identity
			}
			{\loi_exparg\loi_ifempty{\loi_gobarg#1}% 1 seul token ?
				{\ifcat\relax\noexpand#1\expandafter\loi_identity\else\expandafter\loi_gobarg\fi}
				{\loi_identity}% si plusieurs tokens, faux
			}%
		}%
}
\long\def\loi_count_occur#1\in#2:#3{% compte le nombre d'occurrences de #1 dans #2 et met le resultat dans la macro #3
	\long\def\loi_count_occur_a##1##2#1##3\_nil{%
		\loi_ifempty{##3}
			{\def#3{##1}}
			{\expandafter\loi_count_occur_a\number\numexpr##1+1\relax##3\_nil}%
	}%
	\loi_count_occur_a0#2#1\_nil
}
\long\def\loi_check_pair#1#2\in#3{% teste l'appariement de #1 et #2 dans #3
	\loi_ifempty{#3}
		{\loi_second
		}
		{\loi_count_occur#1\in#3:\loi_tempa
		\loi_count_occur#2\in#3:\loi_tempb
		\loi_ifnum{\loi_tempa=\loi_tempb\relax}%
		}%
}
\long\def\loi_grabpaired_expr#1#2#3#4#5{% #1=liste de paires  #2=expression  #3=separateur   #4=resultat    #5=ce qui reste
	\let#4\empty
	\def\loi_remain{#2#3}%
	\loi_foreach\loi_pair\in{#1}{\expandafter\loi_grabpaired_expr_a\loi_pair{#3}#4}%
	\def\loi_remove_lastsep##1#3\_nil{\def#4{##1}}%
	\expandafter\loi_remove_lastsep#4\_nil
	\loi_expafter{\long\def\loi_grab_remain}#4##1\_nil{%
		\loi_ifempty{##1}
			{\let#5\empty}
			{\loi_exparg{\def#5}{\loi_gobarg##1}}%
	}%
	\loi_grab_remain#2\_nil
}
\long\def\loi_grabpaired_expr_a#1#2#3#4{% #1#2=paire en cours  #3=separateur   #4=resultat
	\loi_exparg{\loi_check_pair#1#2\in}#4% si les paires sont appariees dans le resultat
		{}% passer e la paire suivante
		{\long\def\loi_grabpaired_expr_b##1#3##2\_nil{%
			\loi_addtomacro#4{##1#3}% ajouter au resultat ce qui est jusqu'au prochain separateur
			\def\loi_remain{##2}%
			\loi_exparg{\loi_check_pair#1#2\in}{#4}
				{}
				{\loi_ifempty{##2}
					{\loi_error{"\detokenize{#1}" and "\detokenize{#2}" are not paired}}
					{\loi_grabpaired_expr_b##2\_nil}%
				}%
			}%
		\expandafter\loi_grabpaired_expr_b\loi_remain\_nil
		}%
}
\def\insidepair#1#2#3#4{% #1#2=paire  #3=expr  #4=macro reeevant le resultat
	\loi_if_validpair#1#2%
		{\loi_ifcsexpandable{#3}
			{\loi_exparg{\insidepair#1#2}{#3}#4%
			}
			{\loi_check_pair#1#2\in{#3}% si les paires sont appariees dans le resultat
				{\def\insidepair_a##1#1##2\_nil{\insidepair_b##2\_nil{#1}}%
				\def\insidepair_b##1#2##2\_nil##3{%
					\loi_check_pair#1#2\in{##3##1#2}
						{\loi_exparg{\def#4}{\loi_gobarg##3##1}%
						\def\loi_remainafterparen{##2}%
						}%
						{\insidepair_b##2\_nil{##3##1#2}%
						}%
					}%
				\insidepair_a#3\_nil
				}
				{\loi_error{"\detokenize{#1}" and "\detokenize{#2}" are not paired in "#3"}%
				}%
			}%
		}
		{\loi_error{Invalid paired tokens "\detokenize{#1}" and "\detokenize{#2}", empty \string#4 returned}% et bim
		\let#4\empty% voile, bien fait pour vos gueules
		}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%% macro \loi_fornum %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\loi_fornum#1=#2to#3\do{%
	\edef#1{\number\numexpr#2}%
	\expandafter\loi_fornum_a
		\csname loi_fornum_\string#1\expandafter\endcsname\expandafter
		{\number\numexpr#3\expandafter}%
		\expanded{\ifnum#1<\numexpr#3\relax>+\else<-\fi}%
		#1%
}
\long\def\loi_fornum_a#1#2#3#4#5#6{%
	\def#1{%
		\unless\ifnum#5#3#2\relax
			\loi_antefi{#6\edef#5{\number\numexpr#5#41\relax}#1}%
		\fi}%
	#1%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%% macro retirant les espaces extremes %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\long\def\loi_ifspacefirst#1{\expandafter\loi_ifspacefirst_a\detokenize{#10} \_nil}
\long\def\loi_ifspacefirst_a#1 #2\_nil{\loi_ifempty{#1}}
\loi_expafter{\def\loi_gobspace}\space{}
\long\def\loi_removefirstspaces#1{\loi_ifspacefirst{#1}{\loi_exparg\loi_removefirstspaces{\loi_gobspace#1}}{\unexpanded{#1}}}%##BUGFIX v1.63
\begingroup
	\catcode0 12
	\long\gdef\loi_removelastspaces#1{\loi_removelastspaces_a#1^^00 ^^00\_nil}
	\long\gdef\loi_removelastspaces_a#1 ^^00{\loi_removelastspaces_b#1^^00}
	\long\gdef\loi_removelastspaces_b#1^^00#2\_nil{\loi_ifspacefirst{#2}{\loi_removelastspaces_a#1^^00 ^^00\_nil}{\unexpanded{#1}}}
\endgroup
\long\def\loi_removeextremespaces#1{\expanded{\loi_exparg\loi_removelastspaces{\expanded{\loi_removefirstspaces{#1}}}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% macro publique \setsepchar %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\setsepchar{\futurelet\loi_nxttok\setsepchar_a}
\def\setsepchar_a{\loi_ifx{[\loi_nxttok}\setsepchar_b{\setsepchar_b[/]}}
\long\def\setsepchar_b[#1]#2{% #1=sepcar de <liste des sepcar>  #2=<liste des sepcar>
	\loi_ifempty{#1}
		{\loi_error{Empty separator not allowed, separator "/" used}%
		\setsepchar_b[/]{#2}%
		}
		{\def\loi_currentsep{#1}%
		\_removeextremespacesfalse
		\loi_nestcnt1 % reinitaliser niveau initial e 1
		\def\nestdepth{1}%
		\loi_argcsname\let{loi_previndex[\number\loi_nestcnt]}\empty
		\def\loi_listname{loi_listofsep}%
		\let\loi_def\def \let\loi_edef\edef \let\loi_let\let
		\let\loi_listofpair_saved\loi_list_ofpair
		\let\loi_list_ofpair\empty
		\loi_ifempty{#2}
			{\loi_error{Empty list of separators not allowed, "," used}%
			\readlist_g1{,}%
			}
			{\readlist_g1{#2}%
			}%
		\loi_argcsname\let\nestdepth{loi_listofseplen[0]}%
		\loi_argcsname\let\loi_currentsep{loi_listofsep[1]}% 1er car de separation
		\let\loi_listofpair\loi_listofpair_saved
		}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%% macro normalisant l'index %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\loi_normalizeindex#1#2{% #1=macroname  #2=liste d'index  --> renvoie {err}{indx norm}
	\loi_ifempty{#2}
		{{}{}}
		{\loi_exparg{\loi_normalizeindex_a1{}}{\number\csname#1nest\endcsname}{#1}#2,\loi_quark,}%
}%
\def\loi_normalizeindex_a#1#2#3#4#5,{% #1=compteur de profondeur #2=index precedents  #3=profondeur max #4=macroname  #5=index courant
	\loi_ifx{\loi_quark#5}
		{\loi_normalizeindex_c#2\loi_quark% supprimer la derniere virgule
		}
		{\loi_ifnum{#1>#3 }
			{\loi_invalidindex{Too deeply nested index, index [.] retained}{#2}% si profondeur trop grande
			}
			{\loi_ifinrange\ifnum\numexpr#5<0 -1*\fi(#5)[[1:\csname #4len[#20]\endcsname]]% si abs(#5) hors de [1,len]
				{\loi_exparg\loi_normalizeindex_b{\number\numexpr#5\ifnum\numexpr#5<0 +\csname #4len[#20]\endcsname+1\fi}{#1}{#2}{#3}{#4}}
				{\loi_invalidindex{#5 is an invalid index, index [.] retained}{#2}}%
			}%
		}%
}
\def\loi_normalizeindex_b#1#2#3{\loi_exparg\loi_normalizeindex_a{\number\numexpr#2+1}{#3#1,}}% #1=index e rajouter  #2=compteur de profondeur #3=index precedents
\def\loi_normalizeindex_c#1,\loi_quark{{}{#1}}
\def\loi_invalidindex#1#2{\loi_ifempty{#2}{\loi_invalidindex_a{#1},}\loi_invalidindex_a{#1}{#2}}
\def\loi_invalidindex_a#1#2{\loi_invalidindex_b#1\loi_quark#2\loi_quark}
\def\loi_invalidindex_b#1[.]#2\loi_quark#3,\loi_quark#4\loi_quark,{{#1[#3]#2}{#3}}% #4= index ignores

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%% macro publique \readlist %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcount\loi_nestcnt
\def\greadlist{\let\loi_def\gdef\let\loi_edef\xdef\def\loi_let{\global\let}\readlist_a}%
\def\readlist{\let\loi_def\def\let\loi_edef\edef\let\loi_let\let\readlist_a}
\def\readlist_a{%
	\loi_nestcnt1 % niveau initial = 1
	\loi_argcsname\let{loi_previndex[\number\loi_nestcnt]}\empty
	\loi_ifstar{\_removeextremespacestrue\readlist_b}{\_removeextremespacesfalse\readlist_b}%
}
\long\def\readlist_b#1#2{% #1=macro stockant les elements  #2=liste des elements
	\loi_ifcsexpandable{#2}
		{\loi_exparg{\readlist_b#1}{#2}%
		}
		{\loi_edef\loi_listname{\loi_macroname#1}%
		\loi_exparg{\readlist_c#1{#2}}{\loi_listname}%%
		}%
}
\long\def\readlist_c#1#2#3{% #1=macro stockant les elements  #2=liste des elements #3=macroname
	\loi_argcsname\loi_let{#3nest}\nestdepth
	\loi_argcsname\loi_def{#3[]}{#2}% la liste entiere
	\loi_argcsname\loi_def{#3sep[]}{}% separateur vide
	\loi_ifempty{#2}
		{\loi_def#1[##1]{}%
		\loi_argcsname\loi_def{#3len}{0}\loi_argcsname\loi_def{#3len[0]}{0}%
		\loi_error{Empty list ignored, nothing to do}%
		}
		{\loi_def#1[##1]{\expanded{\expandafter\readlist_d\expanded{\loi_normalizeindex{#3}{##1}}{#3}}}%
		\loi_argcsname\loi_def{#3sep}[##1]{\expanded{\expandafter\readlist_d\expanded{\loi_normalizeindex{#3}{##1}}{#3sep}}}%
		\readlist_e{#2}%
		\loi_argcsname\loi_argcsname\loi_let{#3len}{#3len[0]}% longueur du niveau 0
		}%
}
\def\readlist_d#1#2#3{%
	\unexpanded\expandafter\expandafter\expandafter{\csname#3[#2]\expandafter\endcsname\expandafter}%
	\expanded{\loi_ifempty{#1}{}{\unexpanded{\unexpanded{\loi_error{#1}}}}}%
}
\def\readlist_e{%
	\loi_argcsname\loi_let\loi_currentsep{loi_listofsep[\number\loi_nestcnt]}%
	\expandafter\readlist_f\loi_currentsep||\_nil
}
\long\def\readlist_f#1||#2\_nil#3{\readlist_g1{#3#1}}% #1=<sep courant simple>  #3=liste -> rajoute un element vide pour le test \ifempty ci dessous
\long\def\readlist_g#1#2{% #1=compteur d'index  #2=liste d'elements e examiner terminee par <sep courant simple> >>RIEN laisse apres
	\loi_ifempty{#2}
		{\loi_argcsname\loi_edef{\loi_listname len[\csname loi_previndex[\number\loi_nestcnt]\endcsname0]}{\number\numexpr#1-1\relax}%
		\loi_argcsname\loi_let{\loi_listname sep[\csname loi_previndex[\number\loi_nestcnt]\endcsname\number\numexpr#1-1\relax]}\empty% le dernier <sep> est <vide> ##NEW v1.52
		\advance\loi_nestcnt-1
		\loi_argcsname\loi_let\loi_currentsep{loi_listofsep[\number\loi_nestcnt]}%
		}
		{\loi_expafter{\readlist_h{#2}{}}\loi_currentsep||\loi_quark||#2\_nil{#1}% aller isoler le 1er item
		}%
}
\long\def\readlist_h#1#2#3||{% #1=liste restante   #2=<dernier sep utilise>  #3=<sep courant>
	\loi_ifx{\loi_quark#3}% on a epuise tous les <separateurs> ? RESTE e lire <expr+sep1>\_nil{<compteur>}
		{\loi_ifempty{#2}% si #2 vide, aucun <sep utilise> n'a ete trouve, il reste e lire "<liste complete>\_nil"
			{\long\def\readlist_i##1\_nil##2{\loi_exparg{\readlist_j{##2}{}}{\loi_gobarg##1}{#2}}% ##2=compteur d'index
			}
			{\loi_ifx{\loi_listofpair\empty}% paires definies ?
				{\long\def\readlist_i##1#2##2\_nil##3{\loi_exparg{\readlist_j{##3}{##2}}{\loi_gobarg##1}{#2}}%
				}
				{\long\def\readlist_i##1\_nil##2{%
					\loi_exparg{\loi_exparg\loi_grabpaired_expr\loi_listofpair}{\loi_gobarg##1}{#2}\loi_grabpaired_result\loi_grabpaired_remain
					\loi_exparg{\loi_exparg{\readlist_j{##2}}{\loi_grabpaired_remain}}{\loi_grabpaired_result}{#2}}%{#}
				}%
			}%
		\readlist_i\relax% le \relax meuble l'argument delimite
		}
		{\long\def\readlist_i##1#3##2\_nil{%
			\loi_ifempty{##2}% si <liste restante> ne contient pas le <sep courant>
				{\readlist_h{#1}{#2}% recommencer avec le meme <sep utile>
				}%
				{\loi_ifx{\loi_listofpair\empty}% si pas de paires definies
					{\loi_exparg\readlist_h{\loi_gobarg##1#3}{#3}% raccourcir <liste restante> et <sep courant>:=<sep utile>% ##BUGFIX v1.53
					}%
					{\loi_exparg\loi_grabpaired_expr\loi_listofpair{#1#3}{#3}\loi_grabpaired_result\loi_grabpaired_remain
					\loi_ifx{\loi_grabpaired_remain\empty}% si liste non raccourcie #BUGFIX 1.63
						{\loi_exparg\readlist_h{\loi_grabpaired_result}{#2}}% garder le precedent <sep>
						{\loi_exparg\readlist_h{\loi_grabpaired_result}{#3}}%
					}%
				}%
			}%
		\readlist_i\relax#1#3\_nil% ##BUGFIX v1.53
		}%
}
\long\def\readlist_j#1#2#3{% #1=compteur d'index  #2=liste restante  #3=element courant
	\loi_ifnum{0\loi_exparg\loi_ifspacefirst{\loi_currentsep}{}1\if_removeextremespaces1\fi=11 }% s'il faur retirer les espaces extremes
		{\loi_exparg{\loi_exparg{\readlist_k{#1}{#2}}}{\loi_removeextremespaces{#3}}}% redefinir l'element courant
		{\readlist_k{#1}{#2}{#3}}%
}
\long\def\readlist_k#1#2#3#4{% #1=compteur d'index  #2=liste restante  #3=element courant   #4=sep utilise
	\loi_ifnum{0\if_ignoreemptyitems1\fi\loi_ifempty{#3}1{}=11 }
		{\readlist_g{#1}{#2}% si l'on n'ignore pas les elements vides
		}%
		{\loi_argcsname\loi_def{\loi_listname[\csname loi_previndex[\number\loi_nestcnt]\endcsname#1]}{#3}% assignation
		\loi_argcsname\loi_def{\loi_listname sep[\csname loi_previndex[\number\loi_nestcnt]\endcsname#1]}{#4}% assignation du <sep> actuel e la macro \<macrolist>sep
		\loi_ifnum{\loi_nestcnt<\nestdepth\relax}% si imbrication max non atteinte
			{\advance\loi_nestcnt1
			\loi_argcsname\edef{loi_previndex[\number\loi_nestcnt]}{\csname loi_previndex[\number\numexpr\loi_nestcnt-1]\endcsname#1,}%
			\readlist_e{#3}% recommencer avec l'element courant
			}
			{}%
		\loi_exparg\readlist_g{\number\numexpr#1+1}{#2}% puis chercher l'element suivant dans la liste restante
		}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%% macro \listlen %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\listlen#1[#2]{%
	\expanded{%
		\loi_ifempty{#2}
			{\csname\loi_macroname#1len[0]\endcsname}
			{\loi_exparg\listlen_a{\expanded{\loi_macroname#1}}{#2}}%
	}%
}
\def\listlen_a#1#2{% #1=macro name   #2=index non normalise    prendre <profondeur max-1>
	\expandafter\listlen_b\expanded{\loi_normalizeindex{#1}{#2}}{#1}%
}
\def\listlen_b#1#2#3{% #1=err   #2=index normalise  #3=macroname
	\csname#3len[#2,0]\expandafter\endcsname
	\expanded{\loi_ifempty{#1}{}{\unexpanded{\unexpanded{\loi_error{#1}}}}}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% macro \foreachitem %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\foreachitem#1\in#2{%
	\edef\foreachitem_a{\noexpand\foreachitem_c\noexpand#1{\expandafter\noexpand\csname\loi_macroname#1cnt\endcsname}{\loi_macroname#2}}%
	\futurelet\loi_nxttok\foreachitem_b
}
\def\foreachitem_b{\loi_ifx{\loi_nxttok[}\foreachitem_a{\foreachitem_a[]}}
\def\foreachitem_c#1#2#3[#4]{% prendre <profondeur max-1>
	\expandafter\foreachitem_d\expanded{\loi_normalizeindex{#3}{#4}}#1{#2}{#3}%
}
\def\foreachitem_d#1#2{\loi_ifempty{#2}{\foreachitem_e{#1}{}}{\foreachitem_e{#1}{#2,}}}% #1=err  #2=index norm
\long\def\foreachitem_e#1#2#3#4#5#6{% #1=err  #2=index norm  #3=macroiter  #4=compteur associe  #5=nom de macrolist  #6=code
	\loi_ifnum{\csname#5len[#20]\endcsname>0 }
		{\loi_ifempty{#1}{}{\loi_error{#1}}%
		\loi_fornum#4=1to\csname#5len[#20]\endcsname\do{\loi_argcsname\let#3{#5[#2#4]}#6}%
		}
		{}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%% macro \showitem %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\showitems{\loi_ifstar{\let\showitems_cmd\detokenize\showitems_a}{\let\showitems_cmd\loi_identity\showitems_a}}
\def\showitems_a#1{\def\showitems_b{\showitems_d#1}\futurelet\loi_nxttok\showitems_c}
\def\showitems_c{\loi_ifx{\loi_nxttok[}\showitems_b{\showitems_b[]}}
\def\showitems_d#1[#2]{\foreachitem\showitems_iter\in#1[#2]{\showitemsmacro{\expandafter\showitems_cmd\expandafter{\showitems_iter}}}}
\unless\ifdefined\fbox
	\newdimen\fboxrule \newdimen\fboxsep \fboxrule=.4pt \fboxsep=3pt % reglages identiques e LaTeX
	\def\fbox#1{% imitation de la macro \fbox de LaTeX, voir pages 271 e 274 de "Apprendre e programmer en TeX"
		\hbox{%
			\vrule width\fboxrule
			\vtop{%
				\vbox{\hrule height\fboxrule \kern\fboxsep \hbox{\kern\fboxsep#1\kern\fboxsep}}%
				\kern\fboxsep \hrule height\fboxrule
			}\vrule width\fboxrule
		}%
	}
\fi
\def\showitemsmacro#1{% encadrement par defaut
	\begingroup\fboxsep=0.25pt \fboxrule=0.5pt \fbox{\strut#1}\endgroup
	\hskip0.25em\relax
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% macro \itemtomacro %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\itemtomacro#1[#2]{% #1[#2]=item  non encore lu: #3=macro
	\edef\loi_listname{\loi_macroname#1}%
	\expandafter\itemtomacro_a\expanded{\loi_normalizeindex{\loi_listname}{#2}}\let
}
\def\gitemtomacro#1[#2]{% #1[#2]=item
	\xdef\loi_listname{\loi_macroname#1}%
	\expandafter\itemtomacro_a\expanded{\loi_normalizeindex{\loi_listname}{#2}}{\global\let}%
}
\def\itemtomacro_a#1#2#3#4{%
	\loi_ifempty{#1}{}{\loi_error{#1}}%
	\loi_argcsname#3#4{\loi_listname[#2]}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%% reglages par defaut %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\if_removeextremespaces
\newif\if_ignoreemptyitems
\let\ignoreemptyitems\_ignoreemptyitemstrue
\let\reademptyitems\_ignoreemptyitemsfalse
\loi_def_foreachsep{,}
\loi_restorecatcode
\reademptyitems
\setsepchar{,}
\defpair{}
\endinput

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%  historique %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
v1.0    19/8/2016
  - Premiere version publique
----------------------------------------------------------------------
v1.1    01/09/2016
  - Stockage des separateurs dans <macrolist>sep
  - bug corrige dans \loi_restorecatcode
----------------------------------------------------------------------
v1.2    22/10/2016
  - macros \greadlist et \gitemtomacro pour la globalite
----------------------------------------------------------------------
v1.3    18/11/2016
  - bugs corriges dans la gestion de la globalite
----------------------------------------------------------------------
v1.4    05/10/2017
  - test \loi_ifprimitive ajoute au test \loi_ifcs
  - suppression de \loi_expafternil, creation de \loi_expafter,
    modification de \loi_argcsname
  - correction d'un bug : \setsepchar{\par} ne provoque plus d'erreur.
    \loi_ifnum devient \long
----------------------------------------------------------------------
v1.5    06/10/2017
  - correction d'un bug dans \loi_ifcs
----------------------------------------------------------------------
v1.51   24/10/2017
  - correction d'un bug dans \loi_ifcs
----------------------------------------------------------------------
v1.52   13/01/2018
  - le dernier separateur est <vide>
----------------------------------------------------------------------
v1.53   13/03/2018
  - correction d'un bug dans \readlist_i
----------------------------------------------------------------------
v1.6    01/11/2018
  - possibilite d'appariement de tokens dans les items
----------------------------------------------------------------------
v1.61   03/03/2019
  - la macro \loi_ifcs contient une erreur de conception. Il faut
    tester si le token est un sc && s'il est developpable pour
    renvoyer vrai car il existe des sc non developpables && qui ne
    sont _pas_ des primitives.
    Macro rebaptisee \loi_ifcsexpandable
----------------------------------------------------------------------
v1.62   18/05/2019
  - utilisation de la nouvelle primitive \expanded au lieu du
    desormais obsolete \romannumeral
  - bug corrige dans \loi_ifcsexpandable
----------------------------------------------------------------------
v1.63   21/08/2019
  - bug corrige dans \readlist_h avec les tokens apparies
  - bug corrige \loi_removefirstspaces est desormais \long

==> style.tex <==
\usepackage{blindtext}

\usepackage{xcolor, fontawesome}
\definecolor{twitterblue}{RGB}{64,153,255}

\newcommand{\twitter}[1]{\href{https://twitter.com/#1 }{\textcolor{twitterblue}{\faTwitter}\,\tt \textcolor{twitterblue}{#1}}}

\newcommand{\github}[1]{\href{https://github.com/#1 }{\textcolor{black}{\faGithub}\,\tt \textcolor{black}{#1}}}

\newcommand{\tess}{\textit{TESS}}
\newcommand{\sname}{V1298~Tau\xspace}
\newcommand{\allplanets}{V1298~Tau~bcde\xspace}
\newcommand{\planetknown}{V1298~Tau~bcd\xspace}
\newcommand{\planetb}{V1298~Tau~b\xspace}
\newcommand{\planetc}{V1298~Tau~c\xspace}
\newcommand{\planetd}{V1298~Tau~d\xspace}
\newcommand{\planete}{V1298~Tau~e\xspace}
\newcommand{\rearth}{$R_\oplus$\xspace}
\newcommand{\exoplanet}{\texttt{exoplanet}\xspace}


==> xstring.tex <==
% !TeX encoding = ISO-8859-1
% Ce fichier contient le code de l'extension "xstring"
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                    %
\def\xstringname               {xstring}                             %
\def\xstringversion              {1.83}                              %
%                                                                    %
\def\xstringdate              {2019/02/06}                           %
%                                                                    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                    %
% Author     : Christian Tellechea                                   %
% Status     : Maintained                                            %
% Maintainer : Christian Tellechea                                   %
% Email      : unbonpetit@netc.fr                                    %
% Package URL: https://www.ctan.org/pkg/xstring                      %
% Bug tracker: https://framagit.org/unbonpetit/xstring/issues        %
% Repository : https://framagit.org/unbonpetit/xstring/tree/master   %
% Copyright  : Christian Tellechea 2008-2019                         %
% Licence    : Released under the LaTeX Project Public License v1.3c %
%              or later, see http://www.latex-project.org/lppl.txt   %
% Files      : 1) xstring.tex                                        %
%              2) xstring.sty                                        %
%              3) xstring-fr.tex                                     %
%              4) xstring-fr.pdf                                     %
%              5) xstring-en.tex                                     %
%              6) xstring-en.pdf                                     %
%              7) README                                             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifdefined\usepackage\else
	\immediate\write-1 {Package: xstring \xstringdate\space v\xstringversion\space String manipulations (CT)}%
\fi
\newcount\integerpart
\newcount\decimalpart% compteurs utilis?s par xstring

\edef\restorexstringcatcode{\catcode\number`\_ =\number\catcode`\_\relax}
\catcode`\_=11

\long\def\xs_execfirst#1#2{#1}
\long\def\xs_execsecond#1#2{#2}
\long\def\xs_gobarg#1{}
\expandafter\def\expandafter\xs_gobspace\space{}
\def\xs_deftok#1#2{\let#1= #2\relax}\xs_deftok\xs_sptoken{ }
\long\def\xs_ifnxttok#1#2#3{\xs_deftok\xs_toksmatch{#1}\def\__truecode{#2}\def\__falsecode{#3}\xs_ifnxttok_a}
\def\xs_ifnxttok_a{\futurelet\__futurtok\xs_ifnxttok_b}
\def\xs_ifnxttok_b{%
	\xs_ifx{\__futurtok\xs_sptoken}
	{\afterassignment\xs_ifnxttok_a\let\__futurtok= }
	{\xs_ifx{\__futurtok\xs_toksmatch}\__truecode\__falsecode}%
}
\def\xs_ifstar#1{\xs_ifnxttok*{\xs_execfirst{#1}}}
\long\def\xs_testopt#1#2{\xs_ifnxttok[{#1}{#1[{#2}]}}
\long\def\xs_exparg#1#2{\expandafter\xs_exparg_a\expandafter{#2}{#1}}%
\long\def\xs_exparg_a#1#2{#2{#1}}
\long\def\xs_exptwoargs#1#2#3{\xs_exparg{\xs_exparg{#1}{#2}}{#3}}
\long\def\xs_eearg#1#2{\xs_exparg{\xs_exparg{#1}}{#2}}
\long\def\xs_edefaddtomacro#1#2{\edef#1{\unexpanded\expandafter{#1}#2}}
\long\def\xs_addtomacro#1#2{\xs_exparg{\def#1}{#1#2}}
\long\def\xs_eaddtomacro#1#2{\xs_exparg{\xs_addtomacro#1}{#2}}
\long\def\xs_eeaddtomacro#1#2{\xs_exparg{\xs_eaddtomacro#1}{#2}}
\long\def\xs_endgroup_eaddtomacro#1#2{\xs_exparg{\endgroup\xs_addtomacro#1}{#2}}
\long\def\xs_beforespace#1 #2\_nil{#1}
\long\def\xs_afterspace#1 #2\_nil{#2}
\long\def\xs_gobtonil#1\_nil{}
\long\def\xs_gobtobrace#1#{}
\long\def\xs_ifx#1{\ifx#1\expandafter\xs_execfirst\else\expandafter\xs_execsecond\fi}
\def\xs_ifnum#1{\ifnum#1\expandafter\xs_execfirst\else\expandafter\xs_execsecond\fi}
\long\def\xs_ifempty#1{\expandafter\xs_ifx\expandafter{\expandafter\relax\detokenize{#1}\relax}}

\def\xs_toks_toverb{% lit 1 argument et le transforme en verb
\begingroup
\def\do##1{\catcode`##112 }%
\dospecials
\obeyspaces
\xs_read_verb
}

\def\setverbdelim#1{% d?finit quel est le d?limiteur de verb
\xs_exparg\xs_ifempty{\xs_gobarg#1}%
{}
{\errmessage{Package xstring Warning: verb delimiter "\detokenize{#1}" is not a single token}}%
\def\xs_read_verb##1#1##2#1{\endgroup\xs_assign_verb{##2}}% on appelle l'ex?cution de fin
}

% Assigne l'argument entre d?limiteur verb dans la sc #1
\def\verbtocs#1{%
\def\xs_assign_verb##1{\def#1{##1}}%
\xs_toks_toverb
}

\begingroup
\catcode0 3 \gdef\xs_twozeroschars{^^00}%
\catcode0 7 \xdef\xs_twozeroschars{\xs_twozeroschars^^00}%
\endgroup

\edef\xs_reserved_A{\long\def\noexpand\xs_assigntokenizeresult##1\xs_twozeroschars}
\xs_reserved_A#2{\endgroup\xs_exparg{\def#2}{\xs_gobarg#1}}

\def\tokenize#1#2{%
	\begingroup
	\xs_def\xs_reserved_A{#2}% on d?veloppe en accord avec \fullexpandarg ou \noexpandarg
	\everyeof\expandafter{\xs_twozeroschars#1}%
	\endlinechar-1
	\expandafter\xs_assigntokenizeresult\scantokens\expandafter{\expandafter\relax\xs_reserved_A}% on fait l'assignation
}%

\long\def\xs_assign_xstringresult#1#2{\xs_ifempty{#2}{#1}{\def#2{#1}}}

\def\xs_ldef{\long\def}
\def\xs_ledef{\long\edef}

\def\normalexpandarg{%
\let\xs_def\xs_ldef% on d?finit \xs_call avec \def
\def\xs_expand##1{\unexpanded\expandafter{##1}}%
}
\let\noexpandarg\normalexpandarg% synonyme

\def\expandarg{%
\let\xs_def\xs_ldef% on d?finit \xs_call avec \def
\def\xs_expand##1{\unexpanded\expandafter\expandafter\expandafter{##1}}%
}

\def\fullexpandarg{%
\let\xs_def\xs_ledef% on d?finit\xs_call avec \edef
\def\xs_expand##1{##1}% et on neutralise \xs_expand
}

\def\saveexpandmode{\let\xs_saved_def\xs_defarg\let\xs_saved_expand\xs_expand}
\def\restoreexpandmode{\let\xs_defarg\xs_saved_def\let\xs_expand\xs_saved_expand}

% Macro interne renvoyant #2 si son argument commence par une accolade ouvrante "{"
% et #3 sinon (Ulrich Diez sur comp.text.tex)
\long\def\xs_ifbeginwithbrace#1{%
	\csname xs_exec%
	\expandafter\xs_gobarg\string{%
		\expandafter\xs_gobarg\expandafter{\expandafter{\string#1}%
			\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\xs_execfirst
			\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\xs_gobarg
			\expandafter\expandafter\expandafter\xs_gobarg
			\expandafter\expandafter\expandafter{\expandafter\string\expandafter}\string}%
		\expandafter\xs_gobarg\string}%
	\xs_execsecond{first}{second}%
	\endcsname
}

% Cette macro interne prend la 1ere unit? syntaxique de #1 et assigne le r?sultat ? #2
\long\def\xs_returnfirstsyntaxunit#1#2{%
	\let\xs_toks\relax
	\xs_ifempty{#1}
	{\let#2\empty
	}
	{\xs_eearg\xs_ifempty{\expandafter\xs_beforespace\detokenize{#1} \_nil}% #1 commence par un espace ?
		{\def#2{ }}
		{\xs_ifbeginwithbrace{#1}
			{\def\xs_groupfound{\xs_exparg{\def#2}{\expandafter{#2}}\xs_gobtonil}% on met #2 dans des accolades et on finit
				\let\xs_toks\bgroup
				\afterassignment\xs_groupfound
				\def#2%
			}
			{\long\def\xs_assignfirstarg##1##2\_nil{\def#2{##1}}%
				\xs_assignfirstarg
			}%
			#1\_nil
		}%
	}%
}

\long\def\xs_removefirstsyntaxunit#1#2{%
	\xs_ifempty{#1}
	{\let#2\empty
	}
	{\xs_eearg\xs_ifempty{\expandafter\xs_beforespace\detokenize{#1} \_nil}% #1 commence par un espace ?
		{\xs_exparg\xs_ifbeginwithbrace{\xs_gobspace#1}
			{\xs_exparg{\def#2}{\xs_gobtobrace#1}}%
			{\xs_exparg{\def#2}{\xs_afterspace#1\_nil}}%
		}%
		{\xs_exparg{\def#2}{\xs_gobarg#1}}%
	}%
}

% Cette macro interne est utilis?e dans les macros ?toil?es pour :
% 1) d?velopper l'argument selon qu'on a choisit \fullexpandarg
%    ou \normalexpandarg, et ceci ? l'aide de la macro \xs_def
% 2) Ensuite, on d?tokenize ce d?veloppement de fa?on n'avoir plus que
%    des catcodes de 10 pour les espaces et 12 pour le reste.
\long\def\xs_expand_and_detokenize#1#2{%
	\long\def#1{#2}%
	\expandafter\edef\expandafter#1\expandafter{\xs_expand#1}% on d?veloppe #2 selon le mode de d?veloppement
	\long\edef#1{\detokenize\expandafter{#1}}% puis on d?tokenize et on assigne ? #1
}

\long\def\xs_expand_and_assign#1#2{\xs_def#1{#2}}% on d?veloppe #2 selon \fullexpandarg ou \normalexpandarg

\def\xs_arglist{0########1########2########3########4########5########6########7########8########9}

% \xs_assign_args{3} met dans la sc \xs_myarg les tokens "####1####2####3"
\def\xs_assign_args#1{\def\xs_assign_args_i0##1#1##2\_nil{\def\xs_myarg{##1#1}}\expandafter\xs_assign_args_i\xs_arglist\_nil}

% \xs_assign_opt_args{3} met dans la sc \xs_myarg les tokens "[####1]####2####3####4"
\def\xs_assign_opt_args#1{\xs_exparg\xs_assign_opt_args_i{\number\numexpr#1+1}}
\def\xs_assign_opt_args_i#1{\def\xs_assign_opt_args_ii0##11##2#1##3\_nil{\def\xs_myarg{[##11]##2#1}}\expandafter\xs_assign_opt_args_ii\xs_arglist\_nil}

% \xs_assign_one_arg{3} met dans la sc \xs_myarg les tokens "####3"
\def\xs_assign_one_arg#1{\xs_exparg\xs_assign_one_arg_i{\number\numexpr#1-1}{#1}}
\def\xs_assign_one_arg_i#1#2{\def\xs_assign_one_arg_ii##1#1##2#2##3\_nil{\def\xs_myarg{##2#2}}\expandafter\xs_assign_one_arg_ii\xs_arglist\_nil}

% #1 : num?ro du 1er argument; #2 : nombre de lignes; #3 argument optionnel; #4 : dernier num?ro de l'argument devant ?tre d?tokenis? si ?toile
\def\xs_buildlines#1#2#3#4{%
\let\xs_newlines\empty
\let\xs_newargs\empty
\def\xs_buildlines_i##1{%
\xs_exparg\xs_assign_one_arg{\number\numexpr##1+#1-1}%
\edef\xs_reserved_B{\noexpand\xs_expand\csname xs_arg_\romannumeral\numexpr##1\endcsname}%
\xs_ifnum{##1=1 }% si c'est le premier argument
{\xs_ifempty{#3}%
	{\xs_eaddtomacro\xs_newargs{\expandafter{\xs_reserved_B}}%
		\edef\xs_reserved_B{\ifnum##1>#4 xs_def\else xs_assign\fi}%
	}% et s'il y a un argument optionnel alors, on met des crochets
	{\xs_eaddtomacro\xs_newargs{\expandafter[\xs_reserved_B]}%
		\def\xs_reserved_B{xs_def}% ne pas d?tok?niser l'argument optionnel grace au \xs_def
	}%
}
{\xs_eaddtomacro\xs_newargs{\expandafter{\xs_reserved_B}}%
	\edef\xs_reserved_B{\ifnum##1>#4 xs_def\else xs_assign\fi}%
}%
\edef\xs_newlines{\unexpanded\expandafter{\xs_newlines}\expandafter\noexpand\csname\xs_reserved_B\endcsname\expandafter\noexpand\csname xs_arg_\romannumeral\numexpr##1\endcsname{\xs_myarg}}%
\xs_ifnum{##1<#2 }
{\xs_exparg\xs_buildlines_i{\number\numexpr##1+1}}
{}%
}%
\xs_buildlines_i1%
}

\def\xs_newmacro{%
	\xs_ifstar
	{\let\xs_reserved_D\empty\xs_newmacro_}
	{\let\xs_reserved_D\relax\xs_newmacro_0}%
}

% #1 : dernier num?ro de l'argument devant ?tre d?tokenis?
% #2 : nom de la macro publique
% #3 : argument optionnel (vide si pas d'arg optionnel)
% #4 : nombre d'arguments obligatoires
% #5 : utilisation de testopt (1 si oui, 0 si non)
% #6 : code de la macro
\def\xs_newmacro_#1#2#3#4#5{%
	\edef\xs_reserved_A{xs_\expandafter\xs_gobarg\string#2}%
	\edef\xs_reserved_C{\expandafter\noexpand\csname\xs_reserved_A _\ifx\empty#3\empty _\fi\endcsname}%
	\edef\xs_reserved_B{%
		\long
		\ifx\empty\xs_reserved_D
			\def\noexpand#2{\noexpand\xs_ifstar
				{\let\noexpand\xs_assign\noexpand\xs_expand_and_detokenize\expandafter\noexpand\xs_reserved_C}%
				{\let\noexpand\xs_assign\noexpand\xs_expand_and_assign\expandafter\noexpand\xs_reserved_C}%
			}%
		\else
			\def\noexpand#2{\let\noexpand\xs_assign\noexpand\xs_expand_and_assign\expandafter\noexpand\xs_reserved_C}%
		\fi
		\ifx\empty#3\empty
		\else
			\def\expandafter\noexpand\xs_reserved_C{%
				\noexpand\xs_testopt{\expandafter\noexpand\csname\xs_reserved_A __\endcsname}{\ifx\xs_def\xs_ledef#3\else\unexpanded{#3}\fi}}%
		\fi
	}%
	% Que fait \xs_reserved_B ? Il d?finit :
	% si #3 est vide : \NOM{\xs_ifstar{\let\xs_assign\xs_expand_and_detokenize\xs_NOM__}{\let\xs_assign\xs_expand_and_assign\xs_NOM__}}
	% si #3 existe   : \NOM{\xs_ifstar{\let\xs_assign\xs_expand_and_detokenize\xs_NOM_}{\let\xs_assign\xs_expand_and_assign\xs_NOM_}}
	%                  \xs_NOM_{\xs_testopt{\xs_NOM__}{#3}}}
	\xs_reserved_B
	\ifx\empty#3\empty
		\xs_buildlines1{#4}{#3}{#1}%
		\xs_assign_args{#4}%
	\else
		\xs_exparg{\xs_buildlines1}{\number\numexpr#4+1}{#3}{#1}%
		\xs_assign_opt_args{#4}%
	\fi
	\edef\xs_reserved_B{\def\expandafter\noexpand\csname\xs_reserved_A __\endcsname\xs_myarg}%
	\edef\xs_reserved_C{\unexpanded\expandafter{\xs_newlines}\edef\noexpand\xs_call}%
	\edef\xs_reserved_D{\noexpand\noexpand\expandafter\noexpand\csname\xs_reserved_A\endcsname\unexpanded\expandafter{\xs_newargs}}%
	\ifnum#5=1 \edef\xs_reserved_D{\noexpand\noexpand\noexpand\xs_testopt{\unexpanded\expandafter{\xs_reserved_D}}{}}\fi
	\xs_edefaddtomacro\xs_reserved_C{{\unexpanded\expandafter{\xs_reserved_D}}\noexpand\xs_call}%
	\xs_edefaddtomacro\xs_reserved_B{{\unexpanded\expandafter{\xs_reserved_C}}}%
	% Que fait \xs_reserved_B ? Il d?finit par exemple pour 3 arguments obligatoires et 1 facultatif :
	%    \def\xs_NOM__[##2]##3##4##5{%
	%          \xs_def\xs_arg_i{##2}\xs_assign\xs_arg_ii{##3}\xs_assign\xs_arg_iii{##4}\xs_asign\xs_arg_iv{##5}%
	% si #5=0: \edef\xs_call{\noexpand\xs_NOM[\xs_expand\xs_arg_i]{\xs_expand\xs_arg_ii}{\xs_expand\xs_arg_iii}{\xs_expand\xs_arg_iv}}%
	% si #5=1: \edef\xs_call{\noexpand\xs_testopt{\noexpand\xs_NOM[\xs_expand\xs_arg_i]{\xs_expand\xs_arg_i}{\xs_expand\xs_arg_ii}{\xs_expand\xs_arg_iii}{\xs_expand\xs_arg_iv}}{}}%
	%          \xs_call}
	\long\xs_reserved_B
	\edef\xs_reserved_B{%
		\def\expandafter\noexpand\csname\xs_reserved_A\endcsname
		\xs_myarg\ifnum#5=1 [\unexpanded{##}\number\numexpr\ifx\empty#3\empty#4+1\else#4+2\fi]\fi
	}%
	% Que fait \xs_reserved_B ? Il d?finit par exemple pour 3 arguments obligatoires et 1 facultatif :
	%    \def \xs_NOM[##2]##3##4##5[##6]{#6}
	\long\xs_reserved_B
}

% macro g?n?rique qui lit \xs_reserved_C us par us
% 3 sous-routines sont appel?es ? des moments cl? :
% \xs_atendofgroup      (un groupe se finit, appel r?cursif)
% \xs_atbegingroup      (un groupe vient d'?tre ouvert)
% \xs_atnextsyntaxunit  (la future US n'est pas un groupe)
\def\xs_read_reserved_C{%
	\xs_exparg\xs_ifempty{\xs_reserved_C}%
	{\xs_ifnum{\xs_nestlevel=0 }
		{}
		{\xs_atendofgroup
			\xs_read_reserved_C
		}%
	}
	{\xs_exparg\xs_returnfirstsyntaxunit{\xs_reserved_C}\xs_reserved_A
		\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_C}\xs_reserved_C
		\xs_exploregroups
		\xs_ifx{\bgroup\xs_toks}
		{\advance\integerpart1
			\begingroup
			\expandafter\def\expandafter\xs_reserved_C\xs_reserved_A
			\xs_calc_grouIP
			\def\xs_nestlevel{1}%
			\integerpart0
			\xs_atbegingroup
		}
		{\advance\decimalpart1
			\xs_atnextsyntaxunit
		}%
		\xs_read_reserved_C
	}%
}

% macro g?n?rique qui lit \xs_reserved_D en proc?dant ? des tests avec \IfBeginWith
% 1 sous-routine est appel?e :
% \xs_atoccurfound      (une occurrence a ?t? trouv?e)
\def\xs_read_reserved_D{%
	\xs_exparg\xs_ifempty{\xs_reserved_D}%
	{\xs_ifnum{\xs_nestlevel=0 }
		{}
		{\edef\__temp{%
				\endgroup
				\noexpand\decimalpart=\number\decimalpart\relax
				\unexpanded{\xs_addtomacro\xs_reserved_C}{{\unexpanded\expandafter{\xs_reserved_C}}}%
			}%
			\__temp
			\xs_read_reserved_D
		}%
	}%
	{\xs_exptwoargs\xs_IfBeginWith_i\xs_reserved_D\xs_reserved_E
		{\advance\decimalpart1
			\let\xs_reserved_D\xs_reserved_A
			\xs_atoccurfound
		}%
		{\xs_exparg\xs_returnfirstsyntaxunit{\xs_reserved_D}\xs_reserved_A
			\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_D}\xs_reserved_D
			\xs_exploregroups
			\xs_ifx{\bgroup\xs_toks}
			{\advance\integerpart1
				\begingroup
				\expandafter\def\expandafter\xs_reserved_D\xs_reserved_A
				\xs_calc_grouIP
				\let\xs_reserved_C\empty
				\def\xs_nestlevel{1}%
				\integerpart0
			}
			{\xs_eaddtomacro\xs_reserved_C{\xs_reserved_A}%
			}%
		}%
		\xs_read_reserved_D
	}%
}

\xs_newmacro\StrRemoveBraces{}{1}{1}{%
	\def\xs_reserved_C{#1}%
	\let\xs_reserved_B\empty
	\def\xs_nestlevel{0}%
	\xs_StrRemoveBraces_i
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_B}{#2}%
}

\def\xs_StrRemoveBraces_i{%
	\xs_exparg\xs_ifempty{\xs_reserved_C}%
	{\xs_ifnum{\xs_nestlevel=0 }
		{}
		{\xs_endgroup_eaddtomacro\xs_reserved_B\xs_reserved_B
			\xs_StrRemoveBraces_i
		}%
	}
	{\xs_exparg\xs_returnfirstsyntaxunit{\xs_reserved_C}\xs_reserved_A
		\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_C}\xs_reserved_C
		\xs_ifx{\bgroup\xs_toks}
		{\xs_ifx{\xs_exploregroups\relax}% on explore les groupes ?
			{\begingroup
				\expandafter\def\expandafter\xs_reserved_C\xs_reserved_A
				\def\xs_nestlevel{1}%
				\let\xs_reserved_B\empty
			}
			{\expandafter\xs_addtomacro\expandafter\xs_reserved_B\xs_reserved_A
			}%
		}
		{\xs_eaddtomacro\xs_reserved_B{\xs_reserved_A}%
		}%
		\xs_StrRemoveBraces_i
	}%
}

% \xs_cutafteroccur coupe l'argument #1 apr?s la #3?me occurrence de #2
% \xs_reserved_C : contient ce qui se trouve avant cette occurrence
% \xs_reserved_D : contient ce qui se trouve avant cette occurrence y compris cette occurrence
% \xs_reserved_E : contient ce qui se trouve apr?s l'occurrence
% si l'occurrence n'existe pas ou qu'un des arguments est vide, toutes les chaines renvoy?es sont vides
\long\def\xs_cutafteroccur#1#2#3{%
	\xs_ifnum{#3<1 }
	{\let\xs_reserved_C\empty\let\xs_reserved_E\empty\gdef\groupID{}}
	{\xs_cutafteroccur_i{#1}{#2}{#3}}%
}

\long\def\xs_cutafteroccur_i#1#2#3{%
	\def\xs_reserved_D{#1}\let\xs_reserved_C\empty\def\xs_reserved_E{#2}%
	\decimalpart0 \integerpart0 \gdef\groupID{0}\def\xs_nestlevel{0}%
	\def\xs_atoccurfound{%
		\xs_ifnum{\decimalpart=\numexpr(#3)\relax}
		{\edef\__temp{%
				\def\noexpand\xs_reserved_C{\unexpanded\expandafter{\xs_reserved_C}}%
				\def\noexpand\xs_reserved_D{\unexpanded\expandafter{\xs_reserved_D}}%
				\noexpand\decimalpart=\number\decimalpart\relax
			}%
			\expandafter\xs_exitallgroups\__temp
			\xs_gobarg% mange l'appel r?cursif \xs_read_reserved_D dans \xs_read_reserved_D
		}
		{\xs_eaddtomacro\xs_reserved_C{\xs_reserved_E}%
		}%
	}%
	\xs_read_reserved_D
	\xs_ifnum{\decimalpart=\numexpr(#3)\relax}% occurrence trouv?e ?
	{\let\xs_reserved_E\xs_reserved_D
		\xs_exparg{\def\xs_reserved_D}{\xs_reserved_C#2}%
	}
	{\let\xs_reserved_C\empty
		\let\xs_reserved_E\empty
		\gdef\groupID{}%
	}%
}

\xs_newmacro*3\IfSubStr{1}{2}{0}{%
	\xs_cutafteroccur{#2}{#3}{#1}%
	\xs_exparg\xs_ifempty{\xs_reserved_D}\xs_execsecond\xs_execfirst
}

\xs_newmacro*2\IfBeginWith{}{2}{0}{%
	\xs_ifempty{#2}%
	{\xs_execsecond}
	{\xs_IfBeginWith_i{#1}{#2}}%
}

\long\def\xs_IfBeginWith_i#1#2{%
	\xs_ifempty{#2}%
	{\xs_execfirst% #2 est vide, tous les tests sont pass?s avec succ?s : on renvoie #3
	}
	{\xs_ifempty{#1}%
		{\xs_execsecond% #1 est vide, c'est que #2 est + long que #1 : on renvoie #4
		}
		{\xs_returnfirstsyntaxunit{#2}\xs_reserved_B
			\xs_returnfirstsyntaxunit{#1}\xs_reserved_A
			\xs_ifx{\xs_reserved_A\xs_reserved_B}% il y a ?galit?...
			{\xs_removefirstsyntaxunit{#2}\xs_reserved_B
				\xs_removefirstsyntaxunit{#1}\xs_reserved_A% on enl?ve les 1ere unit?s syntaxiques
				\xs_exptwoargs\xs_IfBeginWith_i\xs_reserved_A\xs_reserved_B
			}
			{\xs_execsecond
			}%
		}%
	}%
}

\xs_newmacro*2\IfEndWith{}{2}{0}{%
	\xs_ifempty{#2}%
	{\xs_execsecond
	}
	{\xs_StrCount{#1}{#2}[\xs_reserved_A]%
		\xs_ifnum{\xs_reserved_A=0 }
		{\xs_execsecond}
		{\xs_exparg\xs_ifempty{\xs_reserved_C}}%
	}%
}

\xs_newmacro*4\IfSubStrBefore{1,1}{3}{0}{\xs_IfSubStrBefore_i[#1]{#2}{#3}{#4}}

\def\xs_IfSubStrBefore_i[#1,#2]#3#4#5{%
	\def\xs_reserved_C{#3}%
	\xs_ifx{\xs_exploregroups\relax}% si on explore les groupes
	{\let\xs_reserved_B\empty
		\def\xs_nestlevel{0}%
		\xs_StrRemoveBraces_i% on retire les accolades
		\let\xs_reserved_C\xs_reserved_B
	}
	{}%
	\xs_exparg\xs_cutafteroccur\xs_reserved_C{#5}{#2}%
	\xs_exparg\xs_cutafteroccur\xs_reserved_C{#4}{#1}%
	\gdef\groupID{}%
	\xs_exparg\xs_ifempty{\xs_reserved_C}%
	\xs_execsecond
	\xs_execfirst
}

\xs_newmacro*4\IfSubStrBehind{1,1}{3}{0}{\xs_IfSubStrBehind_i[#1]{#2}{#3}{#4}}
\long\def\xs_IfSubStrBehind_i[#1,#2]#3#4#5{\xs_IfSubStrBefore_i[#2,#1]{#3}{#5}{#4}}

\long\def\xs_formatnumber#1#2{%
	\xs_ifempty{#1}%
	{\def#2{0X}% si vide, renvoie 0X
	}
	{\xs_returnfirstsyntaxunit{#1}\xs_reserved_A
		\def\xs_reserved_B{+}%
		\xs_ifx{\xs_reserved_A\xs_reserved_B}
		{\xs_removefirstsyntaxunit{#1}\xs_reserved_C
			\xs_exparg\xs_ifempty{\xs_reserved_C}%
			{\def#2{+0X}}
			{\xs_exparg{\def#2}{\expandafter+\expandafter0\xs_reserved_C}}%
		}
		{\def\xs_reserved_B{-}%
			\xs_ifx{\xs_reserved_A\xs_reserved_B}
			{\xs_removefirstsyntaxunit{#1}\xs_reserved_A
				\xs_exparg\xs_ifempty{\xs_reserved_A}%
				{\def#2{-0X}}%
				{\xs_exparg{\def#2}{\expandafter-\expandafter0\xs_reserved_A}}%
			}
			{\def#2{0#1}%
			}%
		}%
	}%
}

\xs_newmacro\IfInteger{}{1}{0}{%
	\xs_formatnumber{#1}\xs_reserved_A
	\decimalpart0
	\afterassignment\xs_defafterinteger\integerpart\xs_reserved_A\relax\_nil
	\let\xs_after_intpart\afterinteger
	\expandafter\xs_testdot\afterinteger\_nil
	\xs_ifx{\empty\afterdecimal}
	{\xs_ifnum{\decimalpart=0 }
		{\xs_execfirst% partie d?cimale constitu?e de 0 --> seul cas o? on renvoie vrai
		}
		{\expandafter\xs_defafterinteger\xs_after_intpart\relax\_nil
			\xs_execsecond
		}%
	}
	{\expandafter\xs_defafterinteger\xs_after_intpart\relax\_nil
		\xs_execsecond
	}%
}

\xs_newmacro\IfDecimal{}{1}{0}{%
	\xs_formatnumber{#1}\xs_reserved_A
	\decimalpart0
	\afterassignment\xs_defafterinteger\integerpart\xs_reserved_A\relax\_nil
	\expandafter\xs_testdot\afterinteger\_nil
	\xs_ifx{\empty\afterdecimal}
}

\begingroup\catcode`\@ 11
\long\gdef\xs_defafterinteger#1\relax\_nil{\def\@xs@afterinteger{#1}\let\afterinteger\@xs@afterinteger}
\long\gdef\xs_defafterdecimal#1\_nil{\def\@xs@afterdecimal{#1}\let\afterdecimal\@xs@afterinteger}
\endgroup

\def\xs_testdot{%
\let\xs_decsep\empty
\xs_ifnxttok.
{\def\xs_decsep{.}\xs_readdecimalpart}%
{\xs_testcomma}%
}

\def\xs_testcomma{%
	\xs_ifnxttok,
	{\def\xs_dessep{,}\xs_readdecimalpart}%
		{\xs_defafterdecimal}%
}

\long\def\xs_readdecimalpart#1#2\_nil{%
	\xs_ifempty{#2}
	{\def\xs_reserved_A{0X}}
	{\def\xs_reserved_A{0#2}}%
	\afterassignment\xs_defafterinteger\decimalpart\xs_reserved_A\relax\_nil
	\expandafter\xs_defafterdecimal\afterinteger\_nil
}

% test d'?galit? sur des chaines (et des chaines contenant des nombres)
\long\def\xs_IfStrEqFalse_i#1#2{\let\xs_reserved_A\xs_execsecond}
\long\def\xs_IfStrEqFalse_ii#1#2{% renvoie vrai si les 2 arg sont d?cimaux et s'ils sont ?gaux, faux sinon
	\xs_IfDecimal{#1}%
	{\xs_IfDecimal{#2}%
		{\ifdim#1pt=#2pt
				\let\xs_reserved_A\xs_execfirst
			\else
				\let\xs_reserved_A\xs_execsecond
			\fi% les 2 sont d?cimaux : on fait le test
		}%
		{\let\xs_reserved_A\xs_execsecond}% un seul est d?cimal
	}%
	{\let\xs_reserved_A\xs_execsecond}% #1 n'est pas d?cimal
}

\long\def\xs_TestEqual#1#2{% teste si les 2 arguments sont ?gaux
	\def\xs_reserved_A{#1}\def\xs_reserved_B{#2}%
	\xs_ifx{\xs_reserved_A\xs_reserved_B}
	{\let\xs_reserved_A\xs_execfirst}% ?galit? parfaite des 2 chaines
	{\xs_reserved_D{#1}{#2}}%
	\xs_reserved_A
}

\xs_newmacro*2\IfStrEq{}{2}{0}{% teste si les deux chaines sont ?gales
	\let\xs_reserved_D\xs_IfStrEqFalse_i
	\xs_TestEqual{#1}{#2}%
}

\xs_newmacro*2\IfEq{}{2}{0}{% teste si les 2 arguments (chaine ou nombre) sont ?gaux
	\let\xs_reserved_D\xs_IfStrEqFalse_ii
	\xs_TestEqual{#1}{#2}%
}

\def\IfStrEqCase{%
	\xs_ifstar
	{\xs_IfStringCase{\IfStrEq*}}%
	{\xs_IfStringCase\IfStrEq}%
}

\def\IfEqCase{%
	\xs_ifstar
	{\xs_IfStringCase{\IfEq*}}%
	{\xs_IfStringCase\IfEq}%
}

\long\def\xs_IfStringCase#1#2#3{% #1=macro avec ou sans ?toile  #2=argument ? tester  #3=liste des {<cas>}{code>}
	\long\def\xs_testcase##1##2##3\_nil{% lit les 2 premieres unit?s syntaxiques dans ##1 et ##2. Les autres dans ##3
		#1{#2}{##1}% compare
			{\xs_testopt{\xs_IfStringCase_ii{##2}}{}}% le test est positif, on ex?cute le code correspondant et on mange l'argument optionnel ## BUGfix dans 1.82
			{\xs_ifempty{##3}%
				{\xs_testopt{\xs_IfStringCase_i}{}}% s'il n'y a plus de cas, on ex?cute le code <autres cas> ## BUGfix dans 1.82
				{\xs_testcase##3\_nil}% sinon, on recommence avec ce qui reste
			}%
	}%
	\xs_testcase#3\_nil
}

\long\def\xs_IfStringCase_i[#1]{#1}
\long\def\xs_IfStringCase_ii#1[#2]{#1}

% Renvoie ce qui est ? gauche de l'occurence n?#1 de la sous chaine #3 dans la chaine #2
\xs_newmacro*3\StrBefore{1}{2}{1}{%
	\xs_cutafteroccur{#2}{#3}{#1}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_C}{#4}%
}

% Renvoie ce qui est ? droite de l'occurence n?#1 de la sous chaine #3 dans la chaine #2
\xs_newmacro*3\StrBehind{1}{2}{1}{%
	\xs_cutafteroccur{#2}{#3}{#1}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_E}{#4}%
}

% Renvoie ce qui est strictement compris entre les occurrences n?#1 et n?#2
% des chaines #4 et #5 dans la chaine #3
\xs_newmacro*4\StrBetween{1,1}{3}{1}{\xs_StrBetween_i[#1]{#2}{#3}{#4}[#5]}
\long\def\xs_StrBetween_i[#1,#2]#3#4#5[#6]{%
	\begingroup
	\noexploregroups
	\xs_cutafteroccur{#3}{#5}{#2}%
	\xs_exparg\xs_cutafteroccur{\xs_reserved_C}{#4}{#1}%
	\expandafter
	\endgroup
	\expandafter\xs_assign_xstringresult\expandafter{\xs_reserved_E}{#6}%
	\gdef\groupID{}%
}

\def\exploregroups{\let\xs_exploregroups\relax}
\def\noexploregroups{\def\xs_exploregroups{\let\xs_toks\relax}}
\def\saveexploremode{\let\xs_saveexploremode\xs_exploregroups}
\def\restoreexploremode{\let\xs_exploregroups\xs_saveexploremode}

% Remplace les #1 premi?res occurences de la chaine #3
% par la chaine #4 dans la chaine #2
\xs_newmacro\StrSubstitute{0}{3}{1}{%
	\def\xs_reserved_D{#2}\let\xs_reserved_C\empty\def\xs_reserved_E{#3}%
	\decimalpart0 \integerpart0 \gdef\groupID{0}\def\xs_nestlevel{0}%
	\def\xs_atoccurfound{%
		\xs_ifnum{#1<1 }
		{\def\xs_reserved_A{#4}}
		{\xs_ifnum{\decimalpart>#1 }
			{\def\xs_reserved_A{#3}}
			{\def\xs_reserved_A{#4}}%
		}%
		\xs_eaddtomacro\xs_reserved_C{\xs_reserved_A}%
	}%
	\xs_ifempty{#3}%
	{\xs_exparg\xs_assign_xstringresult{\xs_reserved_D}{#5}%
	}
	{\xs_read_reserved_D
		\xs_exparg\xs_assign_xstringresult{\xs_reserved_C}{#5}%
	}%
}

% Supprime les #1 premi?res occurrences de #3 dans #2
\xs_newmacro\StrDel{0}{2}{1}{\xs_StrSubstitute[#1]{#2}{#3}{}[#4]}

\def\xs_exitallgroups{\ifnum\xs_nestlevel>0 \endgroup\expandafter\xs_exitallgroups\fi}

% Compte combien d'unit?s syntaxiques contient la chaine #1 ?
\xs_newmacro\StrLen{}{1}{1}{%
	\def\xs_reserved_C{#1}\decimalpart0 \def\xs_nestlevel{0}\gdef\groupID{0}%
	\let\xs_atbegingroup\relax
	\def\xs_atendofgroup{\expandafter\endgroup\expandafter\decimalpart\number\decimalpart\relax}%
	\let\xs_atnextsyntaxunit\relax
	\xs_read_reserved_C
	\xs_exparg\xs_assign_xstringresult{\number\decimalpart}{#2}%
}

% Macro interne fermant autant de groupes que n?cessaire pour trouver une unit? syntaxique derri?re
\def\xs_continuetonext{%
	\xs_exparg\xs_ifempty{\xs_reserved_C}%
	{\ifnum\xs_nestlevel>0
			\xs_endgroup_eaddtomacro\xs_reserved_B{\expandafter{\xs_reserved_B}}% on concat?ne
			\expandafter\xs_continuetonext% on recommence
		\fi}
	{}%
}%

\def\xs_calc_grouIP{%
	\begingroup\def\xs_reserved_A{0}%
	\xs_ifx{\xs_reserved_A\groupID}% si on arrive du groupe de niveau 0
	{\endgroup\xdef\groupID{\number\integerpart}}% on met simplement le niveau
	{\endgroup\xs_eearg{\gdef\groupID}{\expandafter\groupID\expandafter,\number\integerpart}}%
}

% Cette macro coupe la chaine #1 apr?s l'unit? syntaxique n?#2
\def\StrSplit{%
	\xs_ifstar
	{\let\xs_reserved_E\xs_continuetonext\StrSplit_i}%
	{\let\xs_reserved_E\relax\StrSplit_i}%
}

\xs_newmacro\StrSplit_i{}{2}{0}{\xs_StrSplit_ii{#2}{#1}\xs_StrSplit_iii}

% Cette macro interne coupe la chaine #2 apr?s l'unit? syntaxique n?#1
% Le d?but est assign? dans \xs_reserved_B et la fin dans \xs_reserved_C
\long\def\xs_StrSplit_ii#1#2{%
	\let\xs_reserved_B\empty\def\xs_reserved_C{#2}\def\xs_reserved_D{#1}\gdef\groupID{}%
	\ifnum#1>0
		\decimalpart0 \integerpart0 \gdef\groupID{0}\def\xs_nestlevel{0}%
		\def\xs_atendofgroup{%
			\edef\__temp{%
				\endgroup
				\noexpand\decimalpart=\number\decimalpart\relax
				\unexpanded{\xs_addtomacro\xs_reserved_B}{{\unexpanded\expandafter{\xs_reserved_B}}}%
			}%
			\__temp
		}%
		\def\xs_atbegingroup{\let\xs_reserved_B\empty}%
		\def\xs_atnextsyntaxunit{%
			\xs_eaddtomacro\xs_reserved_B{\xs_reserved_A}%
			\xs_ifnum{\decimalpart=\xs_reserved_D\relax}
			{\ifx\xs_reserved_C\empty\xs_reserved_E\fi
				\edef\__temp{\def\noexpand\xs_reserved_B{\unexpanded\expandafter{\xs_reserved_B}}\def\noexpand\xs_reserved_C{\unexpanded\expandafter{\xs_reserved_C}}}%
				\expandafter\xs_exitallgroups\__temp
				\xs_gobarg% mange l'appel r?cursif \xs_read_reserved_C dans \xs_read_reserved_C
			}
			{}%
		}%
		\xs_read_reserved_C
	\fi
}

\def\xs_StrSplit_iii#1#2{\let#1\xs_reserved_B\let#2\xs_reserved_C}

% StrCut[n]{<texte>}{<motif>}\macroA\macroB
% \macroA re?oit ce qui se trouve avant la n ?me occurrence <motif> dans <texte>
% \macroB re?oit ce qui est apr?s cette n ?me occurrence
\xs_newmacro*3\StrCut{1}{2}{0}{%
	\xs_ifempty{#3}%
	{\gdef\groupID{}\let\xs_reserved_C\empty\let\xs_reserved_E\empty
	}
	{\xs_ifnum{#1<1 }
		{\xs_StrCut_ii{#2}{#3}1}
		{\xs_StrCut_ii{#2}{#3}{#1}}%
	}%
	\xs_StrCut_iii
}

\long\def\xs_StrCut_ii#1#2#3{%
	\let\xs_reserved_C\empty\def\xs_reserved_D{#1}\def\xs_reserved_E{#2}%
	\decimalpart0 \integerpart0 \gdef\groupID{0}\def\xs_nestlevel{0}%
	\def\xs_atoccurfound{%
		\xs_ifnum{\decimalpart=\numexpr(#3)\relax}
		{\edef\__temp{%
				\def\noexpand\xs_reserved_C{\unexpanded\expandafter{\xs_reserved_C}}%
				\def\noexpand\xs_reserved_D{\unexpanded\expandafter{\xs_reserved_D}}%
				\noexpand\decimalpart=\number\decimalpart\relax
			}%
			\expandafter\xs_exitallgroups\__temp
			\xs_gobarg% stoppe la r?cursivit? dans \xs_read_reserved_D
		}
		{\xs_eaddtomacro\xs_reserved_C{\xs_reserved_E}%
		}%
	}%
	\xs_read_reserved_D
	\let\xs_reserved_E\xs_reserved_D
	\xs_exparg{\def\xs_reserved_D}{\xs_reserved_C#2}%
}

\long\def\xs_StrCut_iii#1#2{\let#1\xs_reserved_C\let#2\xs_reserved_E}

% De la chaine #1, renvoie ce qui se trouve entre les positions
%  #2 et #3, unit?s syntaxiques aux positions compris !
\xs_newmacro\StrMid{}{3}{1}{%
	\begingroup
	\noexploregroups
	\let\xs_reserved_E\relax
	\xs_StrSplit_ii{#3}{#1}%
	\edef\xs_reserved_C{\number\numexpr#2-1}%
	\let\xs_reserved_E\relax
	\xs_exptwoargs\xs_StrSplit_ii\xs_reserved_C\xs_reserved_B
	\expandafter\endgroup
	\expandafter\xs_assign_xstringresult\expandafter{\xs_reserved_C}{#4}%
	\gdef\groupID{}%
}

% supprime #2 unit?s syntaxiques ? gauche dans la chaine #1
\xs_newmacro\StrGobbleLeft{}{2}{1}{%
	\let\xs_reserved_E\relax
	\xs_StrSplit_ii{#2}{#1}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_C}{#3}%
}

% extrait de #1 la chaine ? gauche de longueur #2
\xs_newmacro\StrLeft{}{2}{1}{%
	\let\xs_reserved_E\relax
	\xs_StrSplit_ii{#2}{#1}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_B}{#3}%
}

% supprime #2 unit?s syntaxiques ? droite dans la chaine #1
\xs_newmacro\StrGobbleRight{}{2}{1}{%
	\xs_StrLen{#1}[\xs_reserved_D]%
	\let\xs_reserved_E\relax
	\xs_exparg\xs_StrSplit_ii{\number\numexpr\xs_reserved_D-#2}{#1}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_B}{#3}%
}

% renvoie #2 unit?s syntaxiques ? la droite de la chaine #1
\xs_newmacro\StrRight{}{2}{1}{%
	\xs_StrLen{#1}[\xs_reserved_D]%
	\let\xs_reserved_E\relax
	\xs_exparg\xs_StrSplit_ii{\number\numexpr\xs_reserved_D-#2}{#1}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_C}{#3}%
}

\xs_newmacro\StrChar{}{2}{1}{%
	\let\xs_reserved_B\empty\def\xs_reserved_C{#1}\def\xs_reserved_D{#2}%
	\ifnum#2>0
		\def\groupID{0}\def\xs_nestlevel{0}\integerpart0 \decimalpart0
		\let\xs_atbegingroup\relax
		\def\xs_atendofgroup{\expandafter\endgroup\expandafter\decimalpart\number\decimalpart\relax}%
		\def\xs_atnextsyntaxunit{%
			\ifnum\decimalpart=\xs_reserved_D% la n i?me US est atteinte ?
				\edef\__temp{\def\noexpand\xs_reserved_B{\unexpanded\expandafter{\xs_reserved_A}}}% on capture l'US en cours qui est celle cherch?e
				\expandafter\xs_exitallgroups\__temp
				\expandafter\xs_gobarg% stoppe la r?cursivit? dans \xs_read_reserved_C
			\fi
		}%
		\xs_read_reserved_C
	\fi
	\xs_exparg\xs_ifempty{\xs_reserved_B}%
	{\gdef\groupID{}}
	{}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_B}{#3}%
}

% Combien de fois compte t-on #2 dans #1 ?
\xs_newmacro\StrCount{}{2}{1}{%
	\def\xs_reserved_D{#1}\def\xs_reserved_E{#2}\let\xs_reserved_C\empty
	\xs_ifempty{#2}%
	{\xs_assign_xstringresult{0}{#3}%
	}
	{\decimalpart0 \integerpart0 \gdef\groupID{0}\def\xs_nestlevel{0}%
		\def\xs_atoccurfound{\let\xs_reserved_C\empty\xs_read_reserved_D}%
		\xs_read_reserved_D
		\xs_exparg\xs_assign_xstringresult{\number\decimalpart}{#3}%
	}%
}

% renvoie la position de l'occurrence #1 de la sous chaine #3 dans la chaine #2
\xs_newmacro\StrPosition{1}{2}{1}{%
	\xs_cutafteroccur{#2}{#3}{#1}%
	\let\xs_reserved_E\groupID
	\xs_ifx{\xs_reserved_C\xs_reserved_D}
	{\xs_assign_xstringresult{0}{#4}%
		\let\xs_reserved_E\empty
	}
	{\xs_exparg\xs_StrLen{\xs_reserved_C}[\xs_reserved_C]%
		\xs_exparg\xs_assign_xstringresult{\number\numexpr\xs_reserved_C+1}{#4}%
	}%
	\global\let\groupID\xs_reserved_E
}

\def\comparestrict{\def\xs_comparecoeff{1}}
\def\comparenormal{\def\xs_comparecoeff{0}}
\def\savecomparemode{\let\xs_saved_comparecoeff\xs_comparecoeff}
\def\restorecomparemode{\let\xs_comparecoeff\xs_saved_comparecoeff}

% Compare les deux arguments #1 et #2
% Renvoie 0 s'ils sont ?gaux et renvoie la
% position de la premiere unit? syntaxiques diff?rente sinon
\xs_newmacro*2\StrCompare{}{2}{1}{%
	\def\xs_reserved_A{#1}%
	\def\xs_reserved_B{#2}%
	\xs_ifx{\xs_reserved_B\xs_reserved_A}
	{\xs_assign_xstringresult{0}{#3}}
	{\xs_StrCompare_i{#1}{#2}{#3}}%
}

\long\def\xs_StrCompare_i#1#2#3{%
\def\xs_StrCompare_iii##1{%
\let\xs_reserved_A\empty
\xs_exparg\xs_ifempty{\xs_reserved_C}%
{\edef\xs_reserved_A{*\xs_comparecoeff}}%
{\xs_exparg\xs_ifempty{\xs_reserved_D}%
	{\edef\xs_reserved_A{*\xs_comparecoeff}}
	{}%
}%
\def\xs_next{\xs_exparg\xs_assign_xstringresult{\number\numexpr##1\xs_reserved_A\relax}{#3}}%
}%
\def\xs_StrCompare_ii##1{% ##1 est la position
\xs_exparg\xs_returnfirstsyntaxunit{\xs_reserved_C}\xs_reserved_A
\xs_exparg\xs_returnfirstsyntaxunit{\xs_reserved_D}\xs_reserved_B
\xs_ifx{\xs_reserved_B\xs_reserved_A}
{\xs_exparg\xs_ifempty{\xs_reserved_A}%
	{\xs_StrCompare_iii{##1}% les 2 unit?s syntaxiques sont ?gales, on renvoie la position
	}
	{\def\xs_next{\xs_exparg\xs_StrCompare_ii{\number\numexpr##1+1}}% les 2 unit?s syntaxiques sont ?gales et non vides, on recommence
		\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_C}\xs_reserved_C
		\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_D}\xs_reserved_D
	}%
}% les 2 unit?s syntaxiques sont diff?rentes : on renvoie la position
{\xs_StrCompare_iii{##1}%
}%
\xs_next
}%
\def\xs_reserved_C{#1}\def\xs_reserved_D{#2}%
\xs_StrCompare_ii1%
}

\xs_newmacro\StrFindGroup{}{2}{1}{%
	\def\xs_reserved_A{#2}\def\xs_reserved_B{0}%
	\xs_ifx{\xs_reserved_A\xs_reserved_B}
	{\xs_assign_xstringresult{{#1}}{#3}}
	{\xs_StrFindGroup_i{#1}{#2}[#3]}%
}

\long\def\xs_StrFindGroup_i#1#2[#3]{%
	\def\xs_StrFindGroup_ii{%
		\xs_exparg\xs_ifempty{\xs_reserved_C}%
		{\xs_assign_xstringresult{}{#3}% s'il ne reste plus rien, on renvoie vide
		}
		{\xs_exparg\xs_returnfirstsyntaxunit{\xs_reserved_C}\xs_reserved_D
			\xs_ifx{\bgroup\xs_toks}% si la 1?re unit? syntaxique est un groupe explicite
			{\advance\decimalpart1 % on augmente le compteur
				\xs_ifnum{\decimalpart=\xs_reserved_A\relax}% on est au groupe cherch? lors de la profondeur courante ?
				{\xs_ifx{\empty\xs_reserved_B}% on est ? la profondeur maximale ?
					{\xs_exparg\xs_assign_xstringresult{\xs_reserved_D}{#3}}% on renvoie ce groupe
					{\xs_exparg{\expandafter\xs_StrFindGroup_i\xs_reserved_D}{\xs_reserved_B}[#3]}% on recommence avec ce groupe et les profondeurs de recherche restantes
				}
				{\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_C}\xs_reserved_C
					\xs_StrFindGroup_ii
				}%
			}
			{\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_C}\xs_reserved_C
				\xs_StrFindGroup_ii
			}%
		}%
	}%
	\xs_extractgroupnumber{#2}\xs_reserved_A\xs_reserved_B
	\decimalpart0
	\xs_ifnum{\xs_reserved_A>0 }
	{\def\xs_reserved_C{#1}}
	{\let\xs_reserved_C\empty}%
	\xs_StrFindGroup_ii
}

\def\xs_extractgroupnumber#1#2#3{%
	\def\xs_extractgroupnumber_i##1,##2\_nil{\def#2{##1}\def#3{##2}}%
	\xs_extractgroupnumber_i#1,\_nil
	\ifx\empty#3\else\xs_extractgroupnumber_i#1\_nil\fi
}

\def\expandingroups{\let\xs_expandingroups\exploregroups}

\def\noexpandingroups{\let\xs_expandingroups\noexploregroups}

\def\StrExpand{\xs_testopt{\xs_StrExpand}{1}}
\long\def\xs_StrExpand[#1]#2#3{%
	\begingroup
	\xs_expandingroups
	\xs_ifnum{#1>0 }
	{\integerpart#1 \decimalpart0 \gdef\groupID{0}\def\xs_nestlevel{0}%
		\def\xs_atendofgroup{\xs_endgroup_eaddtomacro\xs_reserved_B{\expandafter{\xs_reserved_B}}}%
		\def\xs_atbegingroup{\let\xs_reserved_B\empty}%
		\def\xs_atnextsyntaxunit{\xs_eeaddtomacro\xs_reserved_B{\xs_reserved_A}}%
		\def\xs_reserved_C{#2}%
		\xs_StrExpand_i{#1}% Appel de la macro r?cursive
	}
	{\def\xs_reserved_B{#2}%
	}
	\expandafter
	\endgroup
	\expandafter\def\expandafter#3\expandafter{\xs_reserved_B}%
	\gdef\groupID{}%
}

\long\def\xs_StrExpand_i#1{%
	\xs_ifnum{#1>0 }
	{\let\xs_reserved_B\empty
		\xs_read_reserved_C
		\let\xs_reserved_C\xs_reserved_B
		\def\xs_reserved_A{\xs_exparg\xs_StrExpand_i{\number\numexpr#1-1}}%
	}
	{\let\xs_reserved_A\relax
	}%
	\xs_reserved_A
}

\def\scancs{\xs_testopt{\xs_scancs}{1}}
\long\def\xs_scancs[#1]#2#3{%
	\xs_StrExpand[#1]{#3}{#2}%
	\edef#2{\detokenize\expandafter{#2}}%
}

\restorexstringcatcode

\setverbdelim{|}%
\fullexpandarg\saveexpandmode
\comparenormal\savecomparemode
\noexploregroups\saveexploremode
\expandingroups

\endinput

H I S T O R I Q U E
------------------------------------------------------------------------------
v1.0    4/7/2008 : - Package achev?.
7/7/2008 : - Package publi? sur CTAN.
------------------------------------------------------------------------------
v1.1    15/8/2008
- Le package ne n?cessite plus LaTeX et est d?sormais utilisable sous
Plain eTeX.
- Ajout des macros \IfInteger et \IfDecimal.
Pour cette derni?re, la partie enti?re et la partie d?cimale sont
r?cup?rables dans les compteurs \integerpart et \decimalpart. Ce
qu'il reste apr?s qu'un caract?re non attendu soit rencontr? est
dispo dans \xs_remainafterdecimal
- Correction d'un bug dans \tokenize :
suppression de l'expansion avec \normalexpandarg pour ?viter le bug
avec les lettres accentu?es dans l'exemple : \tokenize\aa{??}
- Am?lioration du code de la plupart des macros.
- ?criture d'une routine \xs_newmacro d?finissant les  macros.
- Suppression de tous les compteurs grace ? \numexpr.
- Nouvelles fonctionnalit?s internes dans :
\IfSubStr
ajout des chaines se trouvant avant et apr?s l'occurrence test?e
dans les sc \xs_behind_IfSubStr et \xs_before_IfSubStr
\StrCount
a) ajout de ce qui se trouve apr?s la derni?re occurrence dans la
sc \xs_StrCount_afterlastocccur
b) la macro ne d?pend plus d'aucune autre
------------------------------------------------------------------------------
v1.2    23/8/2008
- Am?lioration du code de \StrMid \StrGobbleLeft, \StrLeft,
\StrGobbleRight et \StrRight ? l'aide de la nouvelle macro
\xs_StrSplit_i
- Nouveau test \IfStrEq qui compare 2 chaines
- Nouveau test \IfEq qui compare 2 chaines (ou 2 nombres si les 2 chaines
contiennent un nombre)
- Correction d'un bug dans \xs_formatnumber. La macro n'envisageait pas le
cas o? son argument ?tait vide ce qui faiasait planter
\IfDecimal{}{V}{F} et \IfInteger{}{V}{F}
------------------------------------------------------------------------------
v1.3    21/9/2008
- Am?lioration du code, mise en place de r?cursivit?s terminales dans
toutes les macros r?cursives, simplification de \xs_TestEqual en
utilisant \ifx
- Nouvelles macros \IfStrEqCase et \IfEqCase
Teste si une cha?ne est ?gale ? plusieurs chaines donn?es et
ex?cute un code sp?cifique
- Cr?ation de la macro publique \StrSplit
Coupe la chaine en 2 ? une position donn?e
- Nouvelle macro \StrCompare
Compare 2 cha?nes et renvoie la position du 1er caract?re diff?rent.
Renvoie 0 si elles sont ?gales.
------------------------------------------------------------------------------
v1.3a   29/9/2008
- Correction d'un bug : \expandafter#1
dans les macros \IfSubStrBefore et \StrBetween qui buggue si #1 est un
nombre > 9 !
- R? ?criture de \xs_returnfirstsyntaxunit et \xs_gobarg qui
deviennent purement d?veloppables.
- R? ?criture de \StrLen
- Nouvelle macro interne \xs_cutafteroccur
Coupe la chaine apr?s la ni?me occurrence d'une sous chaine.
- Code am?lior? de \StrMid, \StrLeft, \StrGobbleLeft, \StrRight,
\StrGobbleRight grace ? \xs_cutafteroccur
------------------------------------------------------------------------------
v1.4   4/11/2008
- xstring traite ses arguments par unit? syntaxique, et donc toutes les
macros internes ont ?t? r?-?crites ? cette fin.
- Le manuel a ?t? r?-?crit, rendu plus clair et mieux structur?.
- Nouvelle fonctionnalit? : \expandarg
le 1er lex?me de chaque argument est 1-d?velopp? avant que la
macro ne soit appel?e. Si un argument comporte plus qu'1 lex?me,
il faut passer par \scancs*[1] pour 1-d?velopper toutes les unit?s
syntaxiques.
- Correction de 2 erreurs dans le manuel anglais :  0 est la valeur par
d?faut dans \StrSubstitute et \StrDel
- Coh?rence dans les nom des s?quences de contr?les temporaires qui
sont d?sormais : \xs_reserved_A ? \xs_reserved_E
------------------------------------------------------------------------------
v1.4a  12/11/2008
- Correction d'un bug dans \xs_StrSplit dans le cas o? l'argument
num?rique est <1 : la 1ere coupure doit ?tre vide et le seconde doit
?tre ?gale ? l'argument.
------------------------------------------------------------------------------
v1.4b  16/11/2008
- Correction de 2 bugs dans \xs_returnfirstsyntaxunit
------------------------------------------------------------------------------
v1.5   31/12/2008
- Nouvelles fonctionnalit?s dans la recherche de groupes par un
identificateur caract?risant leur imbrication. Impl?mentation de :
1) \StrFindGroup
2) \groupID
- Ajout des nouvelles macros g?n?riques \xs_read_reserved_C et
\xs_read_reserved_D
- Correction d'un bug dans \StrSplit : \StrSplit{{a}bc}{1}[\truc] faisait
que \truc contenait ?a{a}?.
- Correction d'un bug dans \xs_newmacro : l'argument optionnel ?tait
d?tok?nis? ? tort dans les macros ?toil?es.
- Dans \xs_newmacro, on doit choisir le num?ro du dernier argument devant
?tre d?tok?nis? dans le cas d'une macro ?toil?e (sachant que
l'argument optionnel ne l'est jamais)
------------------------------------------------------------------------------
v1.5a  09/2/2009
- Nouvelle macro \StrExpand, sensible au mode d'exploration. La macro est
ind?pendante du mode d'exploration et dispose de ses propres commandes
d'exploration : \expandingroups et \noexpandingroups
- R?-?criture de \scancs, qui devient triviale puisque d?pendant de
\StrExpand. Il n'y a plus de version ?toil?e et d?sormais, \scancs
est sensible au mode d'exploration.
- Correction d'un bug dans \IfInteger : \IfInteger{2.0}{V}{F} affichait F
- Correction de bugs : mettre \let\xs_reserved_E\relax avant d'appeler
\xs_StrSplit_i
- Suppression des messages d'erreur, de warning et d'info. xstring devient
donc silencieux ;)
- Passage de 3 ? 2 compteurs
- Le manuel est d?sormais plus color?, en esp?rant qu'il sera un peu
plus agr?able ? lire !
------------------------------------------------------------------------------
v1.5b  13/3/2009
- Modification d'un grand nombre de macros de telle sorte que vraiment
n'importe quel code peut d?sormais ?tre plac? dans les arguments des
macros (comme par exemple des \if, \ifx ou autre, m?me sans leur \fi, ce
qui n'?tait pas possible jusqu'alors)
------------------------------------------------------------------------------
v1.5c  05/6/2009
- Correction d'un bug dans \IfBeginWith : il faut appeler
\xs_returnfirstsyntaxunit pour l'argument #2 puis pour l'argument #1 et
non pas l'inverse pour que \xs_toks refl?te ce qui se trouve dans #1
- Correction d'un bug dans \xs_returnfirstsyntaxunit au cas o? #1 commence
par un espace : mettre \xs_toks ? 0
- Correction d'un bug dans \xs_returnfirstsyntaxunit :
\xs_returnfirstsyntaxunit{{}}\truc
faisait que \truc se d?veloppait en un espace.
- Correction d'un bug dans \xs_removefirstsyntaxunit o? le cas
\xs_removefirstsyntaxunit{ {b}}\truc
donnait \truc se d?veloppant en ?b? au lieu de ?{b}?.
------------------------------------------------------------------------------
v1.5d  28/3/2010
- Correction d'un bug dans \IfInteger : \afterinteger ne donnait pas le
bon r?sultat. Par exemple avec 1.23 il renvoyait {} au lieu de {.23}
- \xs_formatnumber ne detokenize plus ses arguments (que m'est-il pass?
par la t?te pour que je code un truc comme ca ?), et donc
\afterinteger et \xs_afterdecimal ont des tokens ayant le bon
catcode
------------------------------------------------------------------------------
v1.6  24/10/2012
- Correction d'un bug dans \xs_cutafteroccur au cas o? #3<1
- \IfDecimal ne \detokenize plus l'argument.
- Nouvelle version de \tokenize qui enlevait les accolades si son argument
?tait entre accolades
- Nouvelle macro \StrCut
- \xs_cutafteroccur_i ne produit plus d'espace ind?sirable si #3 ?tait
?valu? par \numexpr
------------------------------------------------------------------------------
v1.7  13/1/2013
- Correction d'un manque de rigueur dans les assignations concernant
\groupID : elles sont toutes globales d?sormais
- Les macros de xstring sont \long
------------------------------------------------------------------------------
v1.7a 28/2/2013
- Correction d'un espace parasite dans \xs_removefirstsyntaxunit
------------------------------------------------------------------------------
v1.7b 29/7/2013
- La date contenue dans \xstringdate est d?sormais conforme
------------------------------------------------------------------------------
v1.7c 13/10/2013
- les macros impliqu?es dans \IfStrCase et \IfStrEqCase sont d?sormais \long
------------------------------------------------------------------------------
v1.8  07/12/2018
- affectations globales supprim?es (sauf pour \groupID) afin de ne pas
surcharger la pile de sauvegarde
- nettoyage du code, corrections de lourdeurs et maladresses
------------------------------------------------------------------------------
v1.81 09/12/2018
- bug dans \IfInteger et \IfDecimal, la macro \xs_afterdecimal est ind?finie
et doit ?tre remplac?e par \afterdecimal
------------------------------------------------------------------------------
v1.82 01/02/2019
- \xs_testopt n'est pas longue et provoque un bug dans \xs_IfStrCase et
\xs_IfStrCase lorsque #1 contient \par : \xs_testopt reste courte et
\xs_IfStringCase a ?t? modifi?e pour que cela fonctionne.
------------------------------------------------------------------------------
v1.83 06/02/2019
- mauvaise approche et mauvais fix dans la v1.82 : \xs_testopt devient
longue, pas le choix (et donc aussi \xs_ifnxttok)

